Benchmarking the Robustness of Quantized Models

Quantization has emerged as an essential technique for deploying deep neural networks (DNNs) on devices with limited resources. However, quantized models exhibit vulnerabilities when exposed to various noises in real-world applications. Despite the importance of evaluating the impact of quantization on robustness, existing research on this topic is limited and often disregards established principles of robustness evaluation, resulting in incomplete and inconclusive findings. To address this gap, we thoroughly evaluated the robustness of quantized models against various noises (adversarial attacks, natural corruptions, and systematic noises) on ImageNet. Extensive experiments demonstrate that lower-bit quantization is more resilient to adversarial attacks but is more susceptible to natural corruptions and systematic noises. Notably, our investigation reveals that impulse noise (in natural corruptions) and the nearest neighbor interpolation (in systematic noises) have the most significant impact on quantized models. Our research contributes to advancing the robust quantization of models and their deployment in real-world scenarios.

==> src/setup.tex <==
\section{Background and Experimental Setup}

% 模型架构，量化方法，量化比特数，

\subsection{Robustness Evaluation Approaches}

Quantized models that are extensively deployed in edge devices are vulnerable to various perturbations in real-world scenarios. In accordance with the guidelines proposed by Tang \etal \cite{tang2021robustart}, we classify these perturbations into adversarial attacks, natural corruptions, and systematic noises. 

\textbf{Adversarial Attacks}.
To craft the worst-case adversarial perturbations, we employ white-box attacks and set their goals as untargeted misclassification, given that they have complete knowledge of the target model and offer the most substantial attack capabilities.
Subsequently, we provide a brief introduction to the attack methods that we utilize.

- \textbf{Fast Gradient Sign Method (FGSM)}. FGSM \cite{goodfellow2014explaining} is a one-step attack method with $\ell_{\infty}$-norm. 
It calculates the gradient of the loss function with respect to the input only once and subsequently adds gradient noise to generate an adversarial example.
Although FGSM has a relatively weaker attack capability, it is computationally efficient in generating adversarial examples.

- \textbf{Projected Gradient Descent (PGD)}. PGD \cite{madry2017towards} is regarded as one of the most powerful and widely used attacks due to its high attack success rate. It builds upon the FGSM by introducing an iterative process with a gradient projecting at each step. We utilize the PGD attack with different perturbation norms (\ie, PGD-$\ell_{1}$, PGD-$\ell_{2}$, and PGD-$\ell_{\infty}$).

- \textbf{AutoAttack}. Croce \etal \cite{croce2020reliable} proposed two automatic step size adjustment methods (APGD-CE and APGD-DLR) to address problems such as suboptimal step size in PGD. Then they combined two existing complementary attacks to form a parameter-free and computationally affordable attack (\ie, AutoAttack). AutoAttack has demonstrated superior performance compared to state-of-the-art attacks, thus becoming a crucial tool for evaluating model robustness.

 For each attack, we set three different perturbation magnitudes (small, middle, and large). With increasing attack capabilities, these attacks form a progressive evaluation. 

\textbf{Natural Corruptions}.
We employ 15 different perturbation methods from the ImageNet-C benchmark \cite{hendrycks2019benchmarking} to simulate natural corruptions. These methods can be categorized into four groups: (1) noise, which includes \textit{Gaussian noise}, \textit{shot noise}, and \textit{impulse noise}; (2) blur, which includes \textit{defocus blur}, \textit{frosted glass blur}, \textit{motion blur}, and \textit{zoom blur}; (3) weather, which includes \textit{snow}, \textit{frost}, \textit{fog}, and \textit{brightness}; and (4) digital, which includes \textit{contrast}, \textit{elastic}, \textit{pixelation}, and \textit{JPEG compression}. 
Each corruption type is evaluated at five levels of severity to account for variations in the intensity of corruptions. 
Thus, we have 75 perturbation methods in total for natural corruptions evaluation.

\textbf{Systematic Noises}.
In addition, system noises are always present when models are deployed in edge devices due to changes in hardware or software. To simulate these systematic noises, we utilize pre-processing operations from ImageNet-S \cite{wang2021real}. This dataset comprises three frequently used decoders and seven commonly used resize modes. The decoders include implementations from Pillow, OpenCV, and FFmpeg. Meanwhile, the resize operations incorporate bilinear, nearest, cubic, hamming, lanczos, area, and box interpolation modes from the OpenCV and Pillow tools.





\subsection{Quantization Methods}

This paper primarily focuses on Quantization-Aware Training (QAT) methods, which fine-tune quantized models to improve accuracy. Inspired by MQBench \cite{li2021mqbench}, we choose three commonly used quantization methods as follows. Rule-based quantization: DoReFa-Net \cite{zhou2016dorefa}. DoReFa-Net simply clips the activation to $[0,1]$ and then quantizes it, due to the observation that most activation falls into this range in many network architectures (\eg, AlexNet \cite{krizhevsky2017imagenet} and ResNet \cite{he2016deep}). Learning-based quantization: PACT \cite{choi2018pact} and LSQ \cite{esser2019learned}. PACT clips the activation by a handcrafted parameter and optimize the clipping threshold during the backpropagation process. Notice that PACT has no gradient below the clip point, LSQ learns the \textit{scale} alongside network parameters by estimating the gradient at each weight and activation layer. For the choice of quantization bits, we adopt the commonly used set in deployments (\ie, 2, 4, 6, and 8).


\subsection{Architectures and Dataset}
In this work, we apply all quantization methods and robustness evaluation approaches to four architectures, including ResNet18\cite{he2016deep}, ResNet50\cite{he2016deep}, RegNetX600M \cite{radosavovic2020designing}, and MobileNetV2 \cite{sandler2018mobilenetv2}. 
(1) ResNet18 and ResNet50 are popular architectures that use shortcut connections between layers to learn residual functions with reference to the input. And it allows for deeper networks and better performance.
(2) RegNetX600M uses a model structure search method to optimize the network architecture through progressive iteration of the design space.
(3) MobileNetV2 is a lightweight network architecture designed for efficient deployment on edge devices, with depthwise separable convolutions and linear bottlenecks.

Following previous work \cite{li2021mqbench,tang2021robustart}, we evaluate the robustness of quantized models on the ImageNet classification task.  Specifically, we quantize models on the ImageNet train dataset starting from the same floating-point models, and evaluate their robustness using perturbations generated from the ImageNet validation set.

\subsection{Evaluation Metrics}
\textbf{Adversarial Robustness}.
For specific adversarial attacks, we adopt the model accuracy to measure adversarial robustness ($AR$), which is calculated by subtracting the Attack Success Rate (ASR) from 1 (\ie, \textit{$1-ASR$}). The higher $AR$ indicates a stronger model. For the union of different attacks, we adopt the Worst-Case Adversarial Robustness ($WCAR$) to measure the adversarial robustness:
\begin{equation}
WCAR = 1 - P_{(\mathbf{x},\mathbf{y})\sim \mathcal{D}}{\mathrm{Any}(f(\mathcal{A}_{\epsilon,p}^{f}(\mathbf{x})) \neq \mathbf{y}) }, 
\end{equation}
where $f$ is the target model, $\mathcal{A}_{\epsilon,p}$ represents the adversary, $\mathcal{D}$ is the validation set, and $\mathrm{Any}(\cdot)$ is a function that returns true if any of the adversary $\mathcal{A}$ attacks successfully. Similarly, a higher $WCAR$ indicates a stronger model.

\textbf{Natural Robustness}.
We adopt the average accuracy of the quantized model on all natural corruptions to measure natural robustness ($NR$). Formally, we calculate the $NR$ as follows
\begin{equation}
NR = \mathbb{E}_{c\sim C}({P_{(\mathbf{x},\mathbf{y})\sim \mathcal{D}}{(f(c(\mathbf{x}))=\mathbf{y})}}),
\end{equation}
where $c$ denotes a corruption method in the set $C$. A higher value of $NR$ means the quantized model enjoys better natural robustness.


\textbf{Systematic Robustness}.
We adopt the model stability on different systematic noises to measure systematic robustness ($SR$). Specifically, we calculate the standard deviation of accuracy as $SR$:
\begin{equation}
SR = \mathbb{D}_{s\sim S}({P_{(\mathbf{x},\mathbf{y})\sim \mathcal{D}}{(f(s(\mathbf{x}))=\mathbf{y})}}),
\end{equation}
where $s$ denotes a decode or resize method in the set $S$. A lower value of $SR$ means better stability towards different systematic noises.








